Simplicity Bias via Global Convergence of Sharpness Minimization

The remarkable generalization ability of neural networks is usually attributed to the implicit bias of SGD, which often yields models with lower complexity using simpler (e.g. linear) and low-rank features. Recent works have provided empirical and theoretical evidence for the bias of particular variants of SGD (such as label noise SGD) toward flatter regions of the loss landscape. Despite the folklore intuition that flat solutions are 'simple', the connection with the simplicity of the final trained model (e.g. low-rank) is not well understood. In this work, we take a step toward bridging this gap by studying the simplicity structure that arises from minimizers of the sharpness for a class of two-layer neural networks. We show that, for any high dimensional training data and certain activations, with small enough step size, label noise SGD always converges to a network that replicates a single linear feature across all neurons; thereby, implying a simple rank one feature matrix. To obtain this result, our main technical contribution is to show that label noise SGD always minimizes the sharpness on the manifold of models with zero loss for two-layer networks. Along the way, we discover a novel property -- a local geodesic convexity -- of the trace of Hessian of the loss at approximate stationary points on the manifold of zero loss, which links sharpness to the geometry of the manifold. This tool may be of independent interest.

==> gradientdescentmanifold-boundedradius.tex <==
\section{Optimizing a g-convex function in a neighborhood}

\subsection{Decay of the Radius}
First, we show a lemma regarding the gradient of the distance function $d(x_0, x)^2$.
\begin{lemma}\label{lem:gradientofdistancefunction}
    We have
    \begin{align*}
        \nabla_x d(x_0, x)^2 = -\exp^{-1}_x(x_0).
    \end{align*}
\end{lemma}
\begin{proof}
    Consider a curve $\gamma$ starting from $x$, i.e. $\gamma(0) = x$ and initial velocity $v = \gamma'(0)$ for arbitrary $v \in T_x(\mathcal M)$. Then, from the definition of gradient
    \begin{align}
        \Big\langle \nabla_x d(x_0,x)^2, v\Big\rangle = \frac{d}{dt}d(x_0,\gamma(t))^2\Big|_{t=0}.\label{eq:aval}
    \end{align}
    Now look at the distance function $d(x_0, x)^2$ in the tangent space $T_{x_0}(\mathcal M)$. Let $\lambda(t)$ be the pullback of $\gamma$ onto $T_{x_0}(\mathcal M)$ with the exponential map, i.e.
    \begin{align*}
        \lambda(t) = \exp_{x_0}^{-1}(\gamma(t)).
    \end{align*}
    Then, from the definition of differential
    \begin{align*}
        \lambda'(0) = d\exp_{x_0}^{-1}(x)[v].
    \end{align*}
    We can write
    \begin{align*}
        \frac{d}{dt}d(x_0,\gamma(t))^2 = \frac{d}{dt}\|\lambda(t)\|^2 = 2\langle \lambda(t), \lambda'(t) \rangle.
    \end{align*}
    Looking at time zero, we can use the Gauss Lemma to write
    \begin{align}
        \Big\langle \lambda(0), \lambda'(0)\Big\rangle &= \Big\langle d\exp_{x_0}(\lambda(0))[\lambda(0)], d\exp_{x_0}(\lambda(0))[\lambda'(0)]\Big\rangle\\
        &=\Big\langle -\exp_{x}^{-1}(x_0), v\Big\rangle,\label{eq:dovom}
    \end{align}
    where in the second equality we are using the property of the exponential map that
    \begin{align*}
        d\exp_{x_0}(\lambda(0))[\lambda(0)] = d\exp_{x_0}(\exp_{x_0}^{-1}(x))[\exp_{x_0}^{-1}(x)] = -\exp_x^{-1}(x_0).
    \end{align*}
\end{proof}
Comparing Equations~\eqref{eq:aval} and~\eqref{eq:dovom} finishes the proof.
%We can write trace of Hessian     
%    \iffalse
%    \begin{align*}
%        \sum_{j=1}^m\phi({\phi''}^{-1})(w_j) = (y_i)_{i=1}^n,
%    \end{align*}
%    where $\phi({\phi''}^{-1})(w_j)$ means the entrywise application of $\phi({\phi''}^{-1})$ to $w_j$. 
%    \fi

Next, we show that if we evolve according to the gradient flow of some g-convex function $f$ on curve $\gamma(t)$, then the distance of $\gamma$ from the minimizer of $f$ does not increase. 
\begin{lemma}[Decay of the Radius]\label{lem:radiusdecay}
    Suppose $x^*$ is the minimizer of arbitrary smooth function $g$ and $\gamma$ is the solution to the following ODE:
    \begin{align*}
        \frac{d}{dt}\gamma(t) = -\nabla g(\gamma(t)),
    \end{align*}
    where $\nabla$ is the gradient on the manifold. Then, 
    we have
    \begin{align*}
        \frac{d}{dt}d(x^*, \gamma(t))^2 \leq 0. 
    \end{align*}
\end{lemma}
\begin{proof}
    Using Lemma~\ref{lem:gradientofdistancefunction}, defining $w = -\exp^{-1}_{\gamma(t)}(x_0)$, we have
    \begin{align*}
        \frac{d}{dt}d(x_0, \gamma(t))^2 &= \langle w, \gamma'(t)\rangle\\
        &= \langle w, \nabla g(\gamma(t))\rangle\\
        &= \frac{d}{ds}g(\exp_{\gamma(t)}(sw))\Big|_{s=0}.
    \end{align*}
    But note that from g-conveixty of $g$, the function $\exp_{\gamma(t)}(sw)$ is convex in $s$ with minimizer at $s = 1$. Hence, the value of its derivative at zero should be non-positive, which implies
    \begin{align*}
        \frac{d}{dt}d(x_0, \gamma(t))^2 \leq 0.
    \end{align*}
\end{proof}




\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Convexity on the path to optimum]\label{lem:pathconvexity}
    Let $x^*$ be the minimizer of the trace of Hessian of the function $g \triangleq \trace\hess$ on the manifold. Given a point $x$ on the manifold, suppose we know the gradient of $g$ on the manifold is $\delta$-bounded at $x$: $\|\nabla g(x)\| \leq \delta$ for $\delta \leq \sqrt \mu \beta$. Then, the gradient is $\delta$ bounded along the geodesic from $x$ to $x^*$ and $g$ is convex along the geodesic from $x^*$ to $x$. Furthermore, we have
    \begin{align}
        g(x) - g(x^*) \leq \|\nabla g(x)\|d(x^*, x).\label{eq:gradientgapbound}
    \end{align}
\end{lemma}
\begin{proof}
    Suppose $d(x^*,x) = s$ and let $\gamma(t)$ be the unit speed geodesic starting from $\gamma(0) = x^*$ and ending at $\gamma(s) = x$. Then, for any $0\leq t \leq s$ we have
    \begin{align*}
        \frac{d}{dt}\|\nabla g(\gamma(t))\|^2 &= 2\nabla^2 g(\gamma(t))\Big[\gamma'(t),\nabla g(\gamma(t))\Big]\\
        &= 2\nabla^2 g(\gamma(t))\Big[\nabla g(\gamma(t)),\nabla g(\gamma(t))\Big]\\
        &\geq 0,\numberthis\label{eq:derivativeofgradient}
    \end{align*}
    where in the last line we used Lemma~\ref{lem:psdness} to conclude from $\|\nabla g(x)\| \leq \delta$ that the Hessian is PSD on the manifold. 
    The goal is to show that $\|\nabla g(\gamma(t))\| \leq \|\nabla g(\gamma(s))\| < \delta$. To obtain a contradiction, let $0 \leq t_0$ be the supremum of times $t$ for which $\|\nabla g(\gamma(t))\| \geq \delta$ for all $t' \geq t$. Note that $s$ satisfies this condition so $t_0 \leq s$. From the continuity of $\|\nabla g(\gamma(t))\|$, this supermum is actually achieved, namely 
    \begin{align}
        \|\nabla g(\gamma(t_0))\| \geq \delta.\label{eq:avali}
    \end{align}
    Moreover, note that for any $t > t_0$, from Equation~\eqref{eq:derivativeofgradient}
    \begin{align*}
        \frac{d}{dt}\|\nabla g(\gamma(t))\|^2 
        \geq 0,
    \end{align*}
    which implies
    \begin{align*}
        \|\nabla g(\gamma(t))\| \leq \|\nabla g(\gamma(s))\| < \delta.
    \end{align*}
Hence, from continuity of gradient, again we have $\|\nabla g(\gamma(t_0))\| < \delta$. But this contradicts Equation~\eqref{eq:avali}. The contradiction shows that $\|g(\gamma(t))\| < \delta$ along the geodesic from $x^*$ to $x_0$, which from Lemma~\ref{lem:psdness} implies that $g$ is convex along $\gamma(t)$, i.e. it is g-convex as a function of $t$. 
Now define the function $\ell(t) \triangleq g(\gamma(t))$. The $g$-convexity of $g$ along $\gamma(t)$ implies that $\ell$ is convex from zero to $s$, which implies
\begin{align*}
    \ell(0) - \ell(s) \leq \ell'(s)s &= \Big\langle \nabla g(\gamma(s)), \gamma'(s)\Big\rangle s\\
    &\leq -\|\nabla g(\gamma(s))\|s\\
    &= \|\nabla g(x)\|d(x^*, x).
\end{align*}
\end{proof}


\begin{lemma}[Gradient flow decay]
    Along the gradient flow $\frac{d}{dt}\psi(t) = -\nabla g(\psi(t))$ for $g = \trace \hess$ which we know is bounded in a geodesic ball of radius $R$ around $\theta^*$, if $\|\nabla g(\psi(t))\| \leq \delta \leq \sqrt \mu \beta$, we have
    \begin{align*}
        \frac{d}{dt}g(\psi(t)) \leq -[g(\psi(t)) - g(\theta^*)]^2/R^2.
    \end{align*}
\end{lemma}
\begin{proof}
    Note that from the definition of the gradient flow
    \begin{align}
        \frac{d}{dt}g(\psi(t)) = -\|\nabla g(\psi(t))\|^2.\label{eq:aval}
    \end{align}
    On the other hand, from the fact that $\|\nabla g(\psi(t))\| \leq \delta$, Lemma~\ref{lem:pathconvexity} implies 
    \begin{align}
        g(\psi(t)) - g(x^*) \leq \|\nabla g(\psi(t))\|d(\psi(t), x^*) \leq \|\nabla g(\psi(t))\| R.\label{eq:dovom}
    \end{align}
    Combining Equations~\eqref{eq:aval} and~\eqref{eq:dovom} completes the proof.
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%% this theorem is false
\iffalse
\section{Rate of Convergence of Gradient Flow}
\begin{theorem}[Rate of Convergence for gradient flow]
For a $\beta$-normal activation $\phi$ and $\mu$ coherent data gram matrix $X^T X \geq \mu I$ (which also implies $d \geq n$), suppose we start the gradient flow $\psi(t)$ according to the potential $g = \trace \hess$ from $\thetazero$ within radius $R$ (in the manifold distance) from the unique global minimizer of $g$, i.e.
\begin{align*}
    &\psi(0) = \thetazero, \ d(x^*, \thetazero) \leq R,\\
    &\frac{d}{dt}\psi(t) = -\nabla g(\psi(t)).
\end{align*}
Then, the rate of convergence of the gradient flow to the global optimum is upper bounded as
\begin{align*}
        g(\psi(t)) - g(\theta^*) \leq \frac{R^2}{\big[t - (g(\thetazero)/\eta \beta^2)\big]_+ + R^2/g(\thetazero) + R/(\sqrt \eta \beta)},
    \end{align*}
    where $\theta^*$ is the minimizer of the trace of Hessian regularizer on the manifold.
\end{theorem}
\begin{proof}
    First, note that according to Lemma~\ref{lem:radiusdecay} for all $\psi(t)$ we have $d(\psi(t),x^*) \leq R$. Next, note that at any point $\theta$, if $\|\nabla g(\theta)\| \geq \sqrt \eta \beta$, then
    \begin{align}
        \frac{d}{dt} g(\psi(t)) = -\|\nabla g(\psi(t))\|^2 \leq -\eta \beta^2.\label{eq:upperboundone}
    \end{align}
    On the other hand, from Lemma~\ref{lem:radiusdecay}, in case $\|\nabla g(\theta)\| \leq \sqrt \eta \beta$ we have
    \begin{align}
        \frac{d}{dt}g(\psi(t)) \leq -[g(\psi(t)) - g(\theta^*)]^2/R^2.\label{eq:upperboundtwo}
    \end{align}
    Now combining Equations~\eqref{eq:upperboundone} and~\eqref{eq:upperboundtwo} and noting the fact that $g(\theta^*) \geq 0$, we can upper bound $g(\psi(t)) - g(\theta^*)$ with auxiliary function $\rho(t)$ which follows the following ODE
    \begin{align*}
        &\rho(0) = g(\thetazero),\\
        &\frac{d}{dt}\rho(t) = 
        \begin{cases}
        -\eta \beta^2 & \text{if } \rho(t) \geq R\sqrt \eta \beta\\
        -\rho(t)^2/R^2 & \text{otherwise}
        \end{cases}
    \end{align*}
    The solution to this ODE is, if $g(\thetazero) \geq R\sqrt \eta \beta$,
    \begin{align*}
        \rho(t) = 
        \begin{cases}
            g(\thetazero) - t\eta \beta^2 & \text{if } t \geq \frac{g(\thetazero) - R\sqrt \eta \beta}{\eta \beta^2}\\
            \frac{R^2}{t - (g(\thetazero) - R\sqrt \eta \beta)/(\eta \beta^2) + R/(\sqrt \eta \beta)} 
            %= \frac{R^2}{t - g(\thetazero)/(\eta \beta^2) + 2R/(\sqrt \eta \beta)} 
            & \text{otherwise}
        \end{cases}
    \end{align*}
    and if $g(\thetazero) < R\sqrt \eta \beta$,
    \begin{align}
            \rho(t) = \frac{R^2}{t + R^2/g(\thetazero)},
    \end{align}
    which overall can be written as
    \begin{align*}
        \rho(t) \leq \frac{R^2}{\big[t - (g(\thetazero)/\eta \beta^2)\big]_+ + R^2/g(\thetazero) + R/(\sqrt \eta. \beta)}
    \end{align*}
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> motivation.tex <==
\section{Motivation}
We know that in the limit, label noise SGD converge to the gradient flow according to the trace of Hessian of the loss function on the manifold of zero loss. In this work, we investigate under what conditions this gradient flow converges to the minimizer of the trace of Hessian on the manifold of zero loss. We see that under the positivity and strict convexity of the first derivative of the activation $\phi'$ plus an additional normality assumption~\eqref{eq:normalactivation} on the activation function, we can show a $O(1/\epsilon^2)$ rate for convergence of the norm of the gradient below threshold $\epsilon$. Furthermore, if $\phi'$ is strongly convex and has a gap from zero, we can obtain an exponentially fast $O(\log(1/\epsilon))$ rate for convergence of the norm of gradient to zero. Even more, we can translate the smallness of the gradient to proximity of each neuron $\theta_j$ to the optimal neuron $\theta^*_j$ in the subspace spanned by $\{x_i\}_{i=1}^n$ in this regime. The analysis uses a novel geodesic convexity of trace of Hessian on the manifold of zero loss for points $\theta$ where the gradient is small. On the other hand, the norm of the gradient $\|\nabla g\|$ along the gradient flow of $g$ is decreasing even on the manifold for geodesically convex $g$ (Lemma~\ref{}). 

\begin{itemize}
    \item \textbf{Convergence:} For gradient flow we know the value of $f$ converge, but not clear if $\theta$ converge to $\theta^*$. We know under Lojasiewicz inequality, i.e. $|f(\theta_t) - f(\theta^*)|^{1-\alpha}\leq C\|\nabla f(\theta_t)\|$, we get convergence of $\theta_t$ to $\theta^*$ (this probably needs additionally convexity but not sure), but not clear if this condition holds. Under additional smoothness properties of the activations (that we have not assumed) Our problem satisfies
    \begin{align*}
        |f(\theta_t) - f(\theta^*)| \leq C\|\nabla f(\theta_t)\|.
    \end{align*}
    %% see this link: https://angms.science/doc/CVX/GradientFlowConvAna.pdf
    \item 

    
    \item \textbf{Gradient flow on loss in over parameterized linear models: } Authors in~\cite{tarmoun2021understanding} analyze the trajectory of gradient flow in over-parameterized two layer linear networks.
    \item \textbf{Gradient descent avoids strict saddle points: } In~\cite{} authors show that gradient descent with random initialization converges will avoid strict saddle points. However their analysis holds under Lipschitzness of the gradient and is asymptotic.
\end{itemize}



\section{Sketch of the Analysis}
In order to obtain rates for the convergence of the gradient to zero and

Some general points in the analysis.
\begin{itemize}
    \item We show there is only a unique stationary point on the manifold.
    \item We characterize our theory under two general conditions. With\assumpone we show a $O(1/\epsilon^2)$ convergence to $\epsilon$-stationary point on the manifold of zero loss. Notably, this convergence is stronger than the normal $1/\epsilon^2$ convergence rate of gradient descent in the nonconvex optimization literature as there (1) They require the function to be smooth in the sense of optimization while we do not assume any such smoothness on our loss and activations (2) the guarantee holds for one of the points along the trajectory \textbf{Not the last iteration} and (3) the result is defined for functions on Euclidean space not on manifolds. See this paper for such background~\cite{kornowski2021oracle}. In fact the cited paper claims that in the non-smooth case finding $\epsilon$-stationary points in general is impossible. 
    \item Furthermore, under a bit stronger assumption~\assumptwo where the positivity of the first and third derivatives of the activation becomes strict, we show an exponential convergence rate for the Euclidean distance $\|\theta - \theta^*\|$ to the optimal parameter. 
\end{itemize}

Unlike focusing on obtaining a PL or KL inequality for the implicit bias which bounds the optimality gap with the size of the gradient, to argue about the convergence of $\theta$ to $\theta^*$, we bound the distance $\|\theta - \theta^*\|$ with the size of the gradient instead under~\assumptwo.

We show two important properties:
\begin{itemize}
    \item \propone: (Local g-convexity of the implicit regularizer versus Global g-Convexity and PL or KL type inequalities) Note that if the function was $g$-convex, then generalizing the analysis of gradient flow on Euclidean space to manifolds we can show the manifold distance of $\theta$ to $\tehta^*$ goes to zero as well as the suboptimality gap in the objective. However, without convexity, convergence of $\theta$ to $\theta^*$ does not necessarily hold, but under a PL or KL inequality one can show that the objective suboptimality gap goes to zero (exponentially fast in the case of PL inequality). However, this does not say anyting about convergence to $\epsilon$-stationary points without convexity. In fact, we cannot even show a PL or KL inequality for the inmplicit regularizer, but we can show a weaker inequality as the following:
    \[
    f(\theta) - f(\theta^*) \leq C\|\nabla f(\theta)\|,
    \]
    which gives a $O(1/\epsilon)$ rate to reduce the sub-optimality gap by $\epsilon$ for gradient flow but does not imply anything about converging to $\epsilon$ stationary points, e.g. there can be cases where the gradient jump drastically to a large value even after passing long times on the flow.
    \item \paragraph{local-g-convexity versus strict saddle property} Here, we are on manifold so obviously convexity should be generalized to g-convexity, but we cannot get $g$ convexity for the induced regularizer. Instead, we show a weaker local g-convexity around points with small gradient
    under assumption~\assumpone, i.e. we show that for points with small gradient the Hessian of $\trace\hess$ becomes PSD on the manifold. The role that this convexity plays is that it shows the at that point the size of the gradient is non-increasing, hence once the flow reaches a region with small gradient it is trapped there and the algorithm has converged to an $\epsilon$ stationary point. Note that this convexity result can be seen as a stronger condition than claiming the non-existent of non-strict saddle points, which implies convergence for specific types of SGD with symmetric noise, or GD with random initialization in the Euclidean case. The result for GD uses dynamical systems and (1) needs smoothness of the objective (gradient lipschitzness) which we do not assume for our result (2) it depends on random initialization which we don't have guarantee for here (3) is inherently an asymptotic and does not provide epxlicit rate of convergence to stationary points (4) is in the Euclidean space not on manifold~\cite{lee2016gradient}. The results for symmetric noise SGD again require (1) lipschitzness of gradient and Hessian and (2) the dependence of the rate of convergence on these parameters is generally expected to be polynomial but can be quite large (note that we don't even require these Lipschitzness assumptions). Furthermore, 
    \item \paragraph{strong-local-convexity assumption} under~\assumptwo we show for points with small gradient the function becomes strongly g-convex, using which we show an exponential speed for gradient flow to converge to the global minimizer.
    \item Note that we know this g-convexity only locally, i.e. we do not know how to argue it for all the points on the path to the optimum. Therefore, even though we can generalize the typical analysis for gradient descent in the smooth case to the manifold case and in particular show that the point does not exit a geodesic ball with certain radius around the optimum, we cannot do that here due to lack of global convexity.
    \item \paragraph{semi-monotonicity of the gradient and translating smallness of gradient to closeness of $\theta$ to $\theta^*$:} We exploit the structure of our particular optimization problem and show a property we call ``semi-monotonicity" under the slightly stronger assumption on the activation function (\assumptwo), which is similar to the monotonicity of the gradient operator with respect to the optimal point (the norm monotonicity for an operator is similar to strong convexity, i.e. $\langle \nabla f(x) - \nabla f(y), x-y\rangle \geq C\|\theta-\theta^*\|^2$):
    \begin{align*}
        C\|\nabla f(\theta)\| \geq \|\theta - \theta^*\|.
    \end{align*}
    Having this property might create the hope for argueing a type of g-strong convexity for the objective. Nonetheless, note that we do not even have g-convexity all the way on the path to the optimum even if we have local g-convexity at point $\theta$. But combining this property with our local $g$-convexity we show the same type of exponential decay in $\|\theta - \theta^*\|$. This inequality is also similar to PL and Kl inequalities except that the right hand side has been substituted with the actual distance of $\theta$ to $\theta^*$ instead of the suboptimality gap. This semi-monotonicity enables us to translate smallness of the gradient on the manifold to closeness of $\theta$ to $\theta^*$.  
    Furthermore, under~\assumptwo we show a local strong convexity instead of local convexity, which enables us to obtain an exponentially fast rate on the decay of norm of the gradient, which then we translate to an exponentially fast rate on the distance between $\theta$ to $\theta^*$.
\item \paragraph{Gradient remains small, function remains locally-g-convex:} A stregth of our analysis is in the self-feed back loop property that $\epsilon$-stationary and local-g-convexity (or local-strong-g-convexity) properties have; namely, (1) being $\epsilon$ stationary implies being in a locally g-convex region of the manifold, and (2) being in the locally g-convex-region of the manifold implies a non-increasing for the norm of the gradient, which implies that $\theta$ remains an $\epsilon$-stationary point.

\item Even though under Assumption~\ref{assump:one} we get that $\tracehess$ is convex in $\Rr$, it is not necessarily g-convex over the manifold. This is because the Hessian over the manifold is calculated based on the covariant derivative of the manifold, which is different from the Euclidean derivative. In particular, for a hypersurface in Euclidean spsace, the covaraint derivative can be obtained by taking normal Euclidean derivative from the tangent of a curve on the surface, then projecting the resulting vector back onto the tangent space. This operation of projecting back onto the tangent space generates an additional ``projection term" in the algebraic formula of the Hessian of $\tracehess$, which involves the projection operator onto the tangent space. Initially, we observe that it is in general fundamentally difficult to derive analytic estimates for the projection term that relates to the normal Hessian of $\tracehess$ in the Euclidean space. Nonetheless, we discover a novel structure in the manifold of zero loss, which is that even though we cannot prove global g-convexity, but for $\epsilon$-stationary points on the manifold we can relate the projection term of the Hessian of $\tracehess$ on the manifold to the approximate first order optimality condition (equivalently the KKT condition) that we have at an $\epsilon$-stationary point. Using this control on the projection term, we can show that the Hessian of $\tracehess$ is PSD at $\epsilon$ stationary points on the manifold, which implies a weaker local-g-convexity at $\epsilon$ stationary points.
\end{itemize}


==> proofdiscuss.tex <==
%\section{Discussion}

In the literature, other conditions have been used to show convergence (rates) for nonconvex functions. We compare our analysis to those. In particular, in our analysis we prove and exploit a local g-convexity property.
\paragraph{Local g-convexity vs PL inequality: } If a function $F(\theta)$ satisfies a gradient dominance property such as PL (Polyak-Lojasiewicz) or KL inequalities, then one can show the convergence of the gradient flow of $F$ to the global minimum.
%, even though the rate of convergence of $\theta(t)$ to the global minimum is not clear. 
In particular, \citet{damian2021label} show convergence of at least one of the points along the trajectory of SGD somewhere close to a stationary point of $F$ for Label noise SGD, under some assumptions on the loss, including a KL inequality and Lipschitzness of the loss, its gradient, and Hessian. Given a PL or KL inequality, one can prove a bound on the shrinkage of the optimality gap. 

Instead of gradient dominance property, 
    %for which having a gradient dominance inequality can be useful,
    we find the norm of the gradient to be a more effective potential for the landscape of the implicit bias in our setting. This is because once the flow reaches a region with small gradient, the local g-convexity property forces $\|\nabla F\|$ to become non-increasing, hence it gets trapped in the approximate stationary region. Note that this type of convergence is stronger than that in~\cite{damian2021label}, in the sense that it holds for any large enough time.
    
    
    %\item 
    \paragraph{Local g-convexity vs Strict Saddle property:} In this work, we can show the g-convexity property only locally at any approximate stationary point $\theta$.  Hence, we cannot use the argument that $F$ is convex on the geodesic path from $\theta$ to the global optimum $\theta^*$, and the typical convergence analysis of gradient flow in the convex regime is ineffective here.
    
    
    
    %\item \paragraph{local-g-convexity versus strict saddle property} 
    Our local g-convexity can be seen as a stronger property than the non-existence of non-strict saddle points, a popular assumption in the non-convex optimization and deep learning literature~\cite{jin2021nonconvex,allen2020backward}. For instance, a specific variant of SGD whose noise is symmetric enough, or GD with random initialization, can escape strict saddle points in the non-convex landscape~\cite{lee2016gradient,jin2021nonconvex}. Yet, these results are not directly comparable to our setting. Namely, the result for convergence of GD in~\cite{lee2016gradient} (1) uses dynamical systems theory and is inherently asymptotic, (2) needs the objective to be gradient Lipschitz, and (3) crucially depends on the random initialization. Rates for convergence for SGD with specific noise~\cite{jin2021nonconvex} are also typically slow, the convergence is for the best point along the sequence and not for the last time/iterate, and they require Lipschitzness of the gradient. In fact,~\citet{kornowski2021oracle} argue that in the non-smooth case, even finding $\epsilon$-stationary points in general is impossible.  
    %and is not global convergence. 
    Finally, these frameworks have not yet been developed over a manifold which is the focus of this work. In contrast, our argument based on local g-convexity is simple and simply uses the fact that the norm of the gradient becomes non-increasing at approximate stationary points.

